Variance-Reducing Couplings for Random Features

Random features (RFs) are a popular technique to scale up kernel methods in machine learning, replacing exact kernel evaluations with stochastic Monte Carlo estimates. They underpin models as diverse as efficient transformers (by approximating attention) to sparse spectrum Gaussian processes (by approximating the covariance function). Efficiency can be further improved by speeding up the convergence of these estimates: a variance reduction problem. We tackle this through the unifying lens of optimal transport, finding couplings to improve RFs defined on both Euclidean and discrete input spaces. They enjoy theoretical guarantees and sometimes provide strong downstream gains, including for scalable approximate inference on graphs. We reach surprising conclusions about the benefits and limitations of variance reduction as a paradigm, showing that other properties of the coupling should be optimised for attention estimation in efficient transformers.

==> app_save.tex <==
\section{Copulas as a numerical OT solver}
\label{app:copulas}

In this section we provide additional background on Gaussian copulas, as well as the exact details of our experimental setup for the RFF and RLF experiments.
We also provide further discussion on interpretations of coupling random features for GPs, based on \citep{lazaro2010sparse}, and examine whether better kernel approximations improve the accuracy of the associated approximate posterior predictive.

\subsection{Copulas as numerical OT solvers}

\pg{Copulas}
Though an analytic solution remains out of reach, we can nonetheless make progress using a \emph{numerical} OT solver. 
Instead of optimising among the class of \emph{all} joint distributions with prescribed marginals $\Lambda_d(\chi_d)$, we restrict ourselves to a tractable subclass amongst which we can efficiently optimise and sample.
For this, we turn to the statistical tool of \emph{copulas}.
A copula is a multivariate cumulative distribution function (CDF) whose marginals are uniformly distributed on $[0, 1],$ while its joint distribution can be arbitrary.
Given a copula, we can easily enforce the constraint that its marginals are $\chi_d,$ by applying an appropriate CDF, while still retaining necessary flexibility in the joint to reduce estimator variance.
Copulas can be used to model dependencies between random variables and are popular tools in quantitative finance \citep{nelsen2006introduction,haugh2016introduction}.

\pg{Gaussian copulas}
The general family of copulas is still intractable to optimise and sample from, so we constrain ourselves to Gaussian copulas.
These are distributions with uniform marginals whose joint distributions are determined by multivariate Gaussians, as defined below.

\begin{definition}[Gaussian copula]
    Let \smash{$\{\omega_i\}_{i = 1}^m \sim \mathcal{N}(0, \boldsymbol{\Sigma})$} where \smash{$\boldsymbol{\Sigma} \in \mathbb{R}^{m \times m}$} is a correlation matrix, i.e. a positive definite matrix with unit diagonal, and let $F_{\mathcal{N}}$ be the CDF of the standard univariate Gaussian.
    We say $\{F_\mathcal{N}(\omega_i)\}_{i = 1}^m$ is distributed according to a Gaussian copula with covariance $\boldsymbol{\Sigma},$ and use the notation $\{F_\mathcal{N}(\omega_i)\}_{i = 1}^m \sim \text{GC}(\boldsymbol{\Sigma})$ to denote this.
\end{definition}

\pg{Parametrising correlation matrices}
Gaussian copulas are easy to sample from, since they involve only sampling a multivariate Gaussian and applying the univariate Gaussian CDF.
We are therefore left with the task of finding an appropriate correlation matrix $\boldsymbol{\Sigma},$ for which we turn to numerical optimisation.
The family of $m \times m$ correlation matrices can be parameterised by a vector \smash{$\boldsymbol{\theta} \in \mathbb{R}^{m(m - 1) / 2}.$}
In fact, there exist tractable bijections between unconstrained vectors of real numbers \smash{$\boldsymbol{\theta} \in \mathbb{R}^{m(m - 1) / 2}$} and lower triangular Cholesky factors $\mathbf{L}_{\boldsymbol{\theta}}$ such that $\boldsymbol{\Sigma} = \mathbf{L}_{\boldsymbol{\theta}}\mathbf{L}_{\boldsymbol{\theta}}^\top$ is a valid correlation matrix.
In particular, suppose that for each $i = 1, \dots, N,$ and $j = 1, \dots, i,$ we have $\theta_{ij} \in \mathbb{R}^+,$ where $\theta_{ii} = 1.$
Then the parameterisation we use is
\begin{equation}
L_{ij} = \begin{cases}
\frac{\theta_{ij}}{s_i} & \text{ for } i \leq j, \\
0 & \text{ otherwise},
\end{cases}
\end{equation}
where \smash{$s_i = \sqrt{\sum_{j = 1}^i{\theta_{ij}^2}}.$}
Note that, since we are directly parameterising the Cholesky factor, we can sample from the associated Gaussian copula with an $\mathcal{O}(m^2)$ computational cost.

\pg{Optimising correlation matrices}
In order to pick an appropriate correlation matrix $\boldsymbol{\Sigma},$ we optimise it directly to minimise the root mean squared error (RMSE) loss
\begin{equation}
    \label{eq:rmseloss}
    \mathcal{L}(\boldsymbol{\theta}) = \mathbb{E}_{\omega_i}\left[\sqrt{\frac{1}{N^2}\sum_{i, j=1}^N (\phi_{\text{RF}}(\boldsymbol{x}_i)^\top\phi_{\text{RF}}(\boldsymbol{x}_j) - k(\boldsymbol{x}_i, \boldsymbol{x}_j))^2}~\right],
\end{equation}
where $\omega_i \sim \text{GC}(\mathbf{L}_{\boldsymbol{\theta}}\mathbf{L}_{\boldsymbol{\theta}}^\top).$
Note that $\phi_{\text{RF}}$ here depends on $\omega_i,$ though we have suppressed this dependence for simplicity.
Assuming that $\phi_{\text{RF}}$ is differentiable with respect to $\omega_i,$ which is the case in RFFs and RLFs, we can optimise the copula parameters $\boldsymbol{\theta}$ by computing the loss in \cref{eq:rmseloss}, computing its gradients with respect to $\boldsymbol{\theta},$ and updating its values accordingly.

\subsection{Experimental details for RFF and RLF experiments}

\pg{Overview}
In both our RFF and RLF experiments, we compare different coupling schemes for approximating the Gaussian kernel.
The Gaussian kernel, including a lengthscale parameter $\ell,$ an output scale variable $\sigma_v$ and a noise scale parameter $\sigma_n$ takes the form
$$k(x_i, x_j) = \sigma_v^2 \exp\left(-\frac{1}{2 \ell^2} ||\boldsymbol{x}_i - \boldsymbol{x}_j||_2^2\right).$$
Our baselines include standard methods for sampling random frequency vectors for use within RFFs and RLFs, including iid sampling and Halton sequences.
In addition, for both settings, we consider ensembles of frequency vectors that are coupled to have orthogonal directions, but iid lengths.
For a dataset of dimension $d,$ for RFFs we use ensembles of $d$ orthogonal vectors, and for RLFs we use ensembles of $2d$ vectors including $d$ orthogonal basis vectors and their $d$ anti-parallel vectors.

\pg{Selecting kernel hyperparameters}
We want to compare our coupling schemes using realistic kernel hyperparameter values, which we determine as follows.
A realistic application setting for RFFs is within GPs for probabilistic regression.
Therefore, we first fit a GP on a tractable subset of the data, specifically a maximum of 256 randomly chosen datapoints, to select appropriate parameters  $\ell, \sigma_v$ and $\sigma_n.$
We optimise the exact GP marginal likelihood with respect to these hyperparameters, and subsequently fix them.
In RLFs, due to the exponential term in the RLF expression, estimator variance can explode if any sampled frequency $\boldsymbol{\omega}_i$ has even moderately large norm.
To successfully apply RLFs, it is therefore crucial that $\boldsymbol{\omega}_i^\top \boldsymbol{x} < 1$ for essentially all datapoints in the dataset.
More concretely, by \cref{lemma:ot_rff_formulation}, we know that the estimator variance for RLFs depends on $||\boldsymbol{x}_i + \boldsymbol{x}_j||_2,$ and that this quantity must be smaller than $1$ for RLFs to provide reasonable estimates for the Gaussian kernel.
Therefore, we set the lengthscale $\ell$ to two times the average summed norm of the data, namely
$$\ell = 2 \sum_{i,j=1}^N ||\boldsymbol{x}_i + \boldsymbol{x}_j||_2,$$
over the training set.
We train the rest of the kernel parameters, namely $\sigma_v$ and $\sigma_n$ to maximise the marginal likelihood of the data under the exact GP.

\pg{Optimising copula parameters}
In order to learn the copula parameters $\boldsymbol{\theta},$ we optimise $\boldsymbol{\theta}$ on the training set, and then evaluate the quality of the kernel approximation on a test set.

\pg{Splitting procedure}
To obtain mean evaluation metrics and standard errors, we evaluate the methods on multiple random splits as follows.
For each dataset, we conduct cross validation with 20 splits, splitting each dataset into a training and a test set.
Because we train an exact GP to determine kernel hyperparameters, and because we evaluate its predictive NLL, we need to limit the number of datapoints used in both the training and the test set, which we set to a maximum of 256 points each, by sub-sampling at random without replacement.
After training the GP and the copula, we evaluate the metrics on the test set, and repeat this procedure for all 20 splits.

\pg{Optimisation details}
We train both the exact GP as well as the copula using the Adam optimiser \citep{kingma2014adam}, using a learning rate of $10^{-2}.$
The exact GP optimisation stage converges around a thousand steps, and we run it up to $5000$ steps.
The Gaussian copula optimisation stage is highly noisy, since the underlying Gaussian joint is resampled at each step.

\subsection{Do better kernel approximations imply better predictions?}

\pg{Kernel and posterior approximations}
One natural question to ask is whether a better approximation to the kernel function leads to better downstream prediction, e.g.~GP regression.
For example, suppose that, in the GP regression setting, we have drawn an ensemble of frequency vectors with which we define associated random features $\phi_{\text{RF}},$ and group these in a large design matrix $\boldsymbol{\Phi}$ as
\begin{equation}
    \boldsymbol{\Phi}_{ij} = \phi_{\text{RF}}(\boldsymbol{\omega}_i, \boldsymbol{x}_j),
\end{equation}
where we have made the dependence of $\phi_{\text{RF}}$ on $\boldsymbol{\omega}_i$ explicit.
This RF kernel approximation implies an associated linear model, namely 
\begin{equation}
    \boldsymbol{y} = \boldsymbol{w} \boldsymbol{\Phi} + \boldsymbol{\epsilon},
\end{equation}
where $\boldsymbol{w} \sim \mathcal{N}(\boldsymbol{0}, \boldsymbol{I})$ and $\boldsymbol{\epsilon} \sim \mathcal{N}(\boldsymbol{0}, \sigma_n^2\boldsymbol{I}).$
The prior covariance of this linear model is $\boldsymbol{\Phi}^\top \boldsymbol{\Phi}  + \sigma_n^2 \boldsymbol{I},$ which is, by construction, equal in expectation to the exact covariance produced by the kernel, namely $\boldsymbol{K} + \sigma_n^2 \boldsymbol{I}$ by construction.
Now, the predictive means of the approximate linear model are
\begin{align} \label{eq:mua1}
    \boldsymbol{\mu}_{\text{approx}} &= \boldsymbol{\Phi}_p\left(\frac{1}{\sigma_n^2}\boldsymbol{\Phi}_d \boldsymbol{\Phi}_d^\top + \boldsymbol{I}\right)^{-1}\boldsymbol{\Phi}_d\boldsymbol{y}, \\
    \boldsymbol{\mu}_{\text{exact}} &= \boldsymbol{K}_{pd} (\boldsymbol{K}_{dd} + \sigma_n^2 \boldsymbol{I})^{-1}\boldsymbol{y},
\end{align}
and the predictive covariances are
\begin{align} \label{eq:Ca1}
    \boldsymbol{C}_{\text{approx}} &= \boldsymbol{\Phi}_p^\top \left(\frac{1}{\sigma_n^2}\boldsymbol{\Phi}_d \boldsymbol{\Phi}_d^\top + \boldsymbol{I}\right)^{-1} \boldsymbol{\Phi}_p + \sigma_n^2 \boldsymbol{I}, \\
    \boldsymbol{C}_{\text{exact}} &= \boldsymbol{K}_{pp} - \boldsymbol{K}_{pd} (\boldsymbol{K}_{dd} + \sigma_n^2 \boldsymbol{I})^{-1}\boldsymbol{K}_{dp}.
\end{align}
where $\boldsymbol{\Phi}_d$ and $\boldsymbol{\Phi}_p$ are the design matrices corresponding to the training inputs and prediction outputs respectively, $\boldsymbol{K}_{dd}$ is the covariance matrix corresponding the training inputs, $\boldsymbol{K}_{pp}$ is the covariance matrix corresponding to the prediction inputs and $\boldsymbol{K}_{pd}$ and $\boldsymbol{K}_{pd}$ are the cross-covariance matrices between the training and prediction datapoints.
As the number of random features increases, these two models become equal.
But does an improved kernel approximation, via an appropriate coupling scheme, result in more accurate approximations of the predictive mean and covariance?
In our experiments, we have found that this is not necessarily the case.

\pg{Evaluating posterior approximation quality}
As \cref{tab:kld} shows, while the kernel approximation can be improved by using pair-wise norm-coupling, this does not necessarily translate to an improved approximation of the posterior predictive.
In particular, \cref{tab:kld} reports the KL divergence between the exact predictive posterior and the approximate predictive posteriors formed by using either Fourier or Laplace random features.
To elucidate this further we can, instead of \cref{eq:mua1,eq:Ca1} consider writing out the approximate mean and covariance as
\begin{equation} 
    \boldsymbol{\mu}_{\text{exact}} = \tilde{\boldsymbol{K}}_{pd} (\tilde{\boldsymbol{K}}_{dd} + \sigma_n^2 \boldsymbol{I})^{-1}\boldsymbol{y},
    ~~~\boldsymbol{C}_{\text{exact}} = \tilde{\boldsymbol{K}}_{pp} - \tilde{\boldsymbol{K}}_{pd} (\tilde{\boldsymbol{K}}_{dd} + \sigma_n^2 \boldsymbol{I})^{-1}\tilde{\boldsymbol{K}}_{dp},
\end{equation}
where $\tilde{\boldsymbol{K}}_{dd} = \tilde{\boldsymbol{\Phi}}_d^\top \tilde{\boldsymbol{\Phi}}_d,$ 
$\tilde{\boldsymbol{K}}_{pd} = \tilde{\boldsymbol{\Phi}}_d^\top \tilde{\boldsymbol{\Phi}}_p,$ $\tilde{\boldsymbol{K}}_{pd} = \tilde{\boldsymbol{\Phi}}_p^\top \tilde{\boldsymbol{\Phi}}_d$ and $\tilde{\boldsymbol{K}}_{pp} = \tilde{\boldsymbol{\Phi}}_p^\top \tilde{\boldsymbol{\Phi}}_p.$
While introducing pairwise coupling improves the accuracy of our kernel approximation, the approximate mean and covariance also depend on the kernel values through a matrix inverse transformation.
In our experiments, we have found that while pairwise coupling improves the accuracy of $\boldsymbol{\boldsymbol{K}}_{dd}, \boldsymbol{\boldsymbol{K}}_{pd}$ and $\boldsymbol{\boldsymbol{K}}_{pp},$ it did not improve the accuracy of $(\boldsymbol{\boldsymbol{K}}_{dd} + \sigma_n^2 \boldsymbol{I})^{-1},$ and therefore did not improve the overall accuracy of the approximate posterior.

\begin{table}[h!]
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c c}
\toprule
\scshape{Fourier Features} & \scshape{Concrete} & \scshape{Abalone} & \scshape{CPU} & \scshape{Power} & \scshape{Airfoil} & \scshape{Boston} \\
 \midrule
\scshape{IID} & $5.967$ {\tiny $\pm 0.363$} & $0.911$ {\tiny $\pm 0.102$} & $13.887$ {\tiny $\pm 8.971$} & $1.270$ {\tiny $\pm 0.083$} & $4.340$ {\tiny $\pm 0.472$} & $3.416$ {\tiny $\pm 0.378$} \\
\scshape{Halton} & $6.264$ {\tiny $\pm 0.371$} & $0.864$ {\tiny $\pm 0.098$} & $13.733$ {\tiny $\pm 8.817$} & $0.978$ {\tiny $\pm 0.067$} & $4.004$ {\tiny $\pm 0.430$} & $4.013$ {\tiny $\pm 0.433$} \\
\scshape{Orthogonal} & $4.706$ {\tiny $\pm 0.317$} & $0.588$ {\tiny $\pm 0.082$} & $12.808$ {\tiny $\pm 8.308$} & $0.434$ {\tiny $\pm 0.042$} & $3.083$ {\tiny $\pm 0.354$} & $2.759$ {\tiny $\pm 0.283$} \\
\scshape{+ PW Norm-Coupled} & $4.781$ {\tiny $\pm 0.315$} & $0.587$ {\tiny $\pm 0.083$} & $12.919$ {\tiny $\pm 8.331$} & $0.512$ {\tiny $\pm 0.046$} & $3.086$ {\tiny $\pm 0.351$} & $2.769$ {\tiny $\pm 0.284$} \\
 \midrule
\scshape{Laplace Features} & \scshape{Concrete} & \scshape{Abalone} & \scshape{CPU} & \scshape{Power} & \scshape{Airfoil} & \scshape{Boston} \\
 \midrule
\scshape{IID} & $1.487$ {\tiny $\pm 0.106$} & $0.038$ {\tiny $\pm 0.003$} & $1.860$ {\tiny $\pm 0.415$} & $0.151$ {\tiny $\pm 0.007$} & $0.358$ {\tiny $\pm 0.025$} & $2.123$ {\tiny $\pm 0.196$} \\
\scshape{Halton} & $1.542$ {\tiny $\pm 0.104$} & $0.039$ {\tiny $\pm 0.003$} & $1.896$ {\tiny $\pm 0.417$} & $0.137$ {\tiny $\pm 0.006$} & $0.357$ {\tiny $\pm 0.024$} & $2.256$ {\tiny $\pm 0.203$} \\
\scshape{Orthogonal} & $1.164$ {\tiny $\pm 0.113$} & $0.033$ {\tiny $\pm 0.004$} & $1.915$ {\tiny $\pm 0.424$} & $0.029$ {\tiny $\pm 0.002$} & $0.236$ {\tiny $\pm 0.017$} & $1.992$ {\tiny $\pm 0.191$} \\
\scshape{+ PW Norm-Coupled} & $1.163$ {\tiny $\pm 0.112$} & $0.032$ {\tiny $\pm 0.003$} & $1.870$ {\tiny $\pm 0.411$} & $0.029$ {\tiny $\pm 0.002$} & $0.235$ {\tiny $\pm 0.017$} & $1.988$ {\tiny $\pm 0.192$} \\
\bottomrule
\end{tabular}
}
\vspace{1mm}
\caption{
    Kullback-Leibler divergences between exact and approximate GP predictive posterior on held out test sets.
    Divergences are reported in nats.
    Note that we use $d$ features for RFFs and $2d$ features for RLFs.
    Reported errors are equal to two standard errors, i.e. $98\%$ confidence intervals.
}
\label{tab:kld}
\end{table}

==> checklist.tex <==
\newpage
\section{Miscellany: compute, data, impacts and limitations} \label{app:comp_and_impacts}

\pg{Computational resources} 
Our primary contributions are theoretical and conceptual; they need limited computational resources to be verified.
Experiments were carried out on an Intel® Core™ i5-7640X CPU @ 4.00GHz × 4 and a NVIDIA GV102 GPU (rev a1), each requiring 
$< 1$ CPU/GPU hour.


\pg{Datasets and reproducability}
We will make source code publicly available if accepted.
The real-world graphs and meshes were accessed from \cite{community_graphs}, \cite{trimesh} and the online repository published by \citet{borovitskiy2021matern}.
Further information about the datasets is available therein. 
All three repositories were published under the MIT license. 
Where we were able to find them, the original papers introducing the graphs are: \cite{karate,dolphins,polbooks,citeseer,eu-core}.


\pg{Broader impacts}
We envisage several possible impacts of our novel coupled RF algorithms, mostly related to increased scalability.
The improvements to RLFs might unlock better attention approximation in Performers \citep{choromanski2020rethinking}.
Better GRFs might provide similar benefits in graph-based machine learning.
We are particularly excited about our algorithms' possible translational impact in the bioinformatics setting, where datasets are large so efficiency is key.
Coupling RFs is at its heart a technique to improve sampling efficiency so it could also help mitigate the high energy and carbon cost of large models \citep{strubell2019energy}. 
Finally, we believe our results are of intrinsic interest as the first (to our knowledge) rigorously studied application of OT to improving RFs. 
They might spur further research in this domain. 
Our work is foundational; we cannot forsee any immediate direct negative societal impacts. 
However, increases in scalability unlocked by coupled RFs could amplify risks of machine learning, either as unintended consequences or from bad actors.

\pg{Limitations}
We have taken care to detail limitations of our work in the main text, but also summarise them here for the reader's convenience.
First, for RFFs and RLFs the optimality results of Thm.~\ref{thm:pairwise_ot_solution} require assumptions about the number of features $m$ and the data.
Relaxing these is a difficult but important direction for future work. 
For GRFs, we also only coupled $m=2$ walkers and consider walker lengths but not directions. 
More fundamentally, we discuss in Sec.~\ref{sec:discussion} that, despite its ubiquity, variance reduction of pointwise kernel estimates can sometimes be of limited benefit in downstream tasks. 
This more subtle point counters popular assumptions in machine learning and deserves more detailed future study. 


\section{NeurIPS paper checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: All claims in the abstract and introduction are accurately reflected in the main text and appendices.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Assumptions are clearly included in theoretical statements and proofs (see especially the asymptotic assumption in Thm. \ref{thm:pairwise_ot_solution} and the discussion in App. \ref{app:what_are_the_approximations}). 
    The limitations of variance reduction as a broader desideratum for RFs are discussed (see Sec.~\ref{sec:discussion}); this is in fact a key contribution of the paper. 
    See Sec.~\ref{app:comp_and_impacts} for a summary.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: All proofs are (to our knowledge) complete and correct, with assumptions detailed in full.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: All experiments are discussed with ample details of algorithmic implementation. 
    See in particular Apps \ref{app:copulas} and \ref{app:grf_gp_details} for the copula and GP experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: Notwithstanding the fact that our primary contributions are theoretical and conceptual rather than empirical, we will make all code publicly available if the manuscript is accepted.
    Detailed experimental details are provided throughout the text (see especially Secs \ref{app:copulas}, \ref{app:rff_and_rlf_expts} and \ref{app:grf_gp_details}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Details of data splits, hyperparameter optimisation and training are provided in Apps \ref{app:copulas} and \ref{app:grf_gp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All experimental results include standard error estimates. See especially Tables \ref{tab:rff} and \ref{tab:kld} and shaded regions on all plots.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Full details of compute resources are reported in App. \ref{app:comp_and_impacts}. Required resources are limited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: Replace by \answerYes{}
    \item[] Justification: We conform to the code of ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Broader impacts are discussed in App. \ref{app:comp_and_impacts}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our paper presents low to zero risk of misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: Code and datasets are rightly credited in the main text, appendices and bibliography.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: Code will be released if the manuscript is accepted. 
    All details about training, license and limitations will be included.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper involves neither crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper involves neither crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

